Reuse Your Rewards: Reward Model Transfer for Zero-Shot Cross-Lingual Alignment

Aligning language models (LMs) based on human-annotated preference data is a crucial step in obtaining practical and performant LM-based systems. However, multilingual human preference data are difficult to obtain at scale, making it challenging to extend this framework to diverse languages. In this work, we evaluate a simple approach for zero-shot cross-lingual alignment, where a reward model is trained on preference data in one source language and directly applied to other target languages. On summarization and open-ended dialog generation, we show that this method is consistently successful under comprehensive evaluation settings, including human evaluation: cross-lingually aligned models are preferred by humans over unaligned models on up to >70% of evaluation instances. We moreover find that a different-language reward model sometimes yields better aligned models than a same-language reward model. We also identify best practices when there is no language-specific data for even supervised finetuning, another component in alignment.

==> numbers.tex <==
de de 0.9159913659095764
de en 0.7839295268058777
de es 0.8301923871040344
de ru 0.013740300200879574
de tr 0.3713615834712982
de vi 1.923429250717163
en de 1.5038561820983887
en en 1.315834403038025
en es 1.0129140615463257
en ru 0.024423882365226746
en tr 0.8270952701568604
en vi 3.3049497604370117
es de 1.777888536453247
es en 1.6331013441085815
es es 1.510971188545227
es ru 0.09928300976753235
es tr 1.393092155456543
es vi 3.923593521118164
ru de 0.7895684242248535
ru en 0.4497399628162384
ru es 0.45829808712005615
ru ru 0.017082899808883667
ru tr 0.3625759482383728
ru vi 1.2588297128677368
tr de 2.198126792907715
tr en 1.9137606620788574
tr es 1.8256258964538574
tr ru 0.1508876383304596
tr tr 1.3356387615203857
tr vi 4.280564308166504
vi de 1.7849547863006592
vi en 2.5181093215942383
vi es 1.7354400157928467
vi ru 0.022210462018847466
vi tr 1.4663113355636597
vi vi 4.368443489074707


==> results.tex <==
KLs
seahorse
src tgt kl
de de 0.9159913659095764
de en 0.7839295268058777
de es 0.8301923871040344
de ru 0.013740300200879574
de tr 0.3713615834712982
de vi 1.923429250717163
en de 1.5038561820983887
en en 1.315834403038025
en es 1.0129140615463257
en ru 0.024423882365226746
en tr 0.8270952701568604
en vi 3.3049497604370117
es de 1.777888536453247
es en 1.6331013441085815
es es 1.510971188545227
es ru 0.09928300976753235
es tr 1.393092155456543
es vi 3.923593521118164
ru de 0.7895684242248535
ru en 0.4497399628162384
ru es 0.45829808712005615
ru ru 0.017082899808883667
ru tr 0.3625759482383728
ru vi 1.2588297128677368
tr de 2.198126792907715
tr en 1.9137606620788574
tr es 1.8256258964538574
tr ru 0.1508876383304596
tr tr 1.3356387615203857
tr vi 4.280564308166504
vi de 1.7849547863006592
vi en 2.5181093215942383
vi es 1.7354400157928467
vi ru 0.022210462018847466
vi tr 1.4663113355636597
vi vi 4.368443489074707

